Data-Driven Evidence-Based Syntactic Sugar Design

Programming languages are essential tools for developers, and their evolution plays a crucial role in supporting the activities of developers. One instance of programming language evolution is the introduction of syntactic sugars, which are additional syntax elements that provide alternative, more readable code constructs. However, the process of designing and evolving a programming language has traditionally been guided by anecdotal experiences and intuition. Recent advances in tools and methodologies for mining open-source repositories have enabled developers to make data-driven software engineering decisions. In light of this, this paper proposes an approach for motivating data-driven programming evolution by applying frequent subgraph mining techniques to a large dataset of 166,827,154 open-source Java methods. The dataset is mined by generalizing Java control-flow graphs to capture broad programming language usages and instances of duplication. Frequent subgraphs are then extracted to identify potentially impactful opportunities for new syntactic sugars. Our diverse results demonstrate the benefits of the proposed technique by identifying new syntactic sugars involving a variety of programming constructs that could be implemented in Java, thus simplifying frequent code idioms. This approach can potentially provide valuable insights for Java language designers, and serve as a proof-of-concept for data-driven programming language design and evolution.

==> temp.tex <==
Frequent pattern mining has been well explored in software engineering research. Frequent pattern mining has been used to mine API elements which appear together in source code \cite{Michail00ICSEAssociation, LiPrMiner}. Later works improve upon these techniques by mining API pairs (i.e, method calls commonly performed together) \cite{WasylkowskiAnomalies, EnglerInferringErrors, YangPerracotta, WeimerTemporalErrors}. Other works have mined and analyzed frequent change patterns \cite{NegaraCodeChanges, DilharaPythonChanges, RefactoringMiner1.0, RefactoringMiner2.0} and used frequent patterns to detect code clones \cite{QianClones, BasitClones}. Most similar to our approach, \cite{NguyenGrouMiner} mines partial orders from source code. Broadly, these previous works involve the mining of API usages, refactoring classification, or code clone detection to improve developer productivity, discover defects, and increase code quality. No previous works consider mining the frequent usages of a programming language's features to motivate data-driven programming language evolution through syntactic sugars. This task involves unique challenges such as balancing the removal of project-specific information with modeling repetition and duplication, meanwhile preserving the context of the represented idioms.

%----------------------------------------------------------------------------------

Researchers have applied frequent pattern mining techniques to provide insights into repetitive patterns in open-source repositories. Works such as GrouMiner~\cite{NguyenGrouMiner} have leveraged these techniques to discover common object protocols and detect anomalies. \citet{NegaraCodeChanges} applied frequent pattern mining to extract frequent code change patterns, resulting in the discovery of 11 previously unknown patterns.

In the area of code refactorings, \citet{BritoJavaRefactorings} characterized non-trivial subgraphs representing refactorings in Java and Javascript applications, while \citet{JankeTSECodeChange} mined version control systems to extract 25 frequent change patterns found across multiple software projects. 

\citet{QianClones} and \citet{BasitClones} have applied frequent subgraph mining to the area of code clone detection. The identification of various degrees of code clones and code clone snippets can assist in software maintenance. Therefore, \citet{BasitClones} uses an approach to discover design-level similarities, and \citet{QianClones} mines an enriched model to detect logical structure clones.

Our approach of generalizing a graph representation of source code builds upon previous works that have found that removing irrelevant elements and modifying the representation can expedite the analysis and produce more meaningful results \cite{UpadhyayaAccel, AllenStaged, ChoiSparseDataFlow, SmaragdakisSetBased}. Similarly, our use of a simplified control-flow graph to extract frequent subgraphs and motivate new syntactic sugars for Java programming language is inspired by works like \citet{YamaguchiCodePropGraphs}, which proposed a code property graph for discovering common vulnerabilities.

%----------------------------------------------------------------------------------


